Enabling Cost-Effective UI Automation Testing with Retrieval-Based LLMs: A Case Study in WeChat

UI automation tests play a crucial role in ensuring the quality of mobile applications. Despite the growing popularity of machine learning techniques to generate these tests, they still face several challenges, such as the mismatch of UI elements. The recent advances in Large Language Models (LLMs) have addressed these issues by leveraging their semantic understanding capabilities. However, a significant gap remains in applying these models to industrial-level app testing, particularly in terms of cost optimization and knowledge limitation. To address this, we introduce CAT to create cost-effective UI automation tests for industry apps by combining machine learning and LLMs with best practices. Given the task description, CAT employs Retrieval Augmented Generation (RAG) to source examples of industrial app usage as the few-shot learning context, assisting LLMs in generating the specific sequence of actions. CAT then employs machine learning techniques, with LLMs serving as a complementary optimizer, to map the target element on the UI screen. Our evaluations on the WeChat testing dataset demonstrate the CAT's performance and cost-effectiveness, achieving 90% UI automation with $0.34 cost, outperforming the state-of-the-art. We have also integrated our approach into the real-world WeChat testing platform, demonstrating its usefulness in detecting 141 bugs and enhancing the developers' testing process.

==> motivation.tex <==
\section{Industrial Motivation}
\label{sec:motivation}
Large Language Models (LLMs) introduce a new era in a wide range of tasks.
It mainly refers to the Transformer-based~\cite{vaswani2017attention} language models that are trained on ultra-large-scale corpora, such as GPT~\cite{brown2020language}, PaLM~\cite{chowdhery2022palm}, LLaMA~\cite{touvron2023llama}, T5~\cite{raffel2020exploring}, etc.
These models exhibit capabilities that are not present in
smaller models, including program synthesis~\cite{li2023cctest}, and multi-step reasoning~\cite{wei2022chain}.
% Large Language Models (LLMs), such as ChatGPT [42], GPT-4 [43], PaLM [7], and LLaMA [55], are trained on ultra-large-scale corpora and can support a wide range of tasks with prompt engineering.
Specifically, the input of LLMs is a natural language prompt, LLMs can be invoked to generate the responses and perform specific tasks without requiring additional training or hard coding.



Yet, applying LLMs for UI automation in the industry involves two main challenges, including cost optimization and knowledge integration. 
First, while there are many works that focus on using LLMs for UI automation~\cite{?}, it is costly, which may not be affordable for industry-level testing.
According to~\cite{web:openaiprice}, the price of querying ChatGPT API [42] is \$3 / 1000K tokens.
% , worsely the UI representation (i.e., view hierarchy) is usually lengthy (about 40k tokens on average for each UI).
Even if we can deploy a private LLM service, the computational cost is still high. 
For example, inferring a single token with LLaMA-7B~\cite{touvron2023llama} takes 6.7 billion FLOPs, and the whole process of UI automation may use over 2,000 tokens.
Second, LLMs lack knowledge and experience about certain apps, especially for industry apps.
This is because, concerning license copyright violations arising from the LLMs~\cite{web:copyright}, the training does not contain industry resources.
Figure 2 shows an example where a deep understanding of the industrial app is needed to complete the task. 
It is difficult to determine solely based on semantics and prior knowledge that clicking on ‘more options’ and then ’settings’ on the first two screens will lead to the screen containing the option to ‘delete all events’.


% Taken in this sense, it is worthwhile developing a new effective method to optimize UI automation for industrial apps.
% To integrate industrial app knowledge, a common paradigm is in-context learning~\cite{?} by few-shot examples.
% By augmenting the prompt with a few examples of industrial app usage, LLMs can understand, analyze, organize, and produce desired outputs for UI automation.

